Reed's conjecture on some special classes of graphs

Reed conjectured that for any graph $G$, $\chi(G) \leq \lceil \frac{\omega(G)+\Delta(G)+1}{2}\rceil$, where $\chi(G)$, $\omega(G)$, and $\Delta(G)$ respectively denote the chromatic number, the clique number and the maximum degree of $G$. In this paper, we verify this conjecture for some special classes of graphs, in particular for subclasses of $P_5$-free graphs or $Chair$-free graphs.

==> ChairHouseBullDartKite.tex <==
% Generated with LaTeXDraw 2.0.8
% Sat Mar 31 11:30:07 CEST 2012
% \usepackage[usenames,dvipsnames]{pstricks}
% \usepackage{epsfig}
% \usepackage{pst-grad} % For gradients
% \usepackage{pst-plot} % For axes
\begin{figure}[t]
\scalebox{1} % Change this value to rescale the drawing.
{
\begin{pspicture}(0,-0.83640623)(8.005938,0.79640627)
\psdots[dotsize=0.1](0.386875,0.7264063)
\psdots[dotsize=0.1](0.386875,0.22640625)
\psdots[dotsize=0.1](0.386875,-0.27359375)
\psdots[dotsize=0.1](0.886875,0.22640625)
\psdots[dotsize=0.1](0.886875,-0.27359375)
\psline[linewidth=0.03cm](0.886875,0.22640625)(0.886875,-0.27359375)
\psline[linewidth=0.03cm](0.386875,0.22640625)(0.886875,0.22640625)
\psline[linewidth=0.03cm](0.386875,0.7264063)(0.386875,-0.27359375)
\psdots[dotsize=0.1](1.986875,-0.27359375)
\psdots[dotsize=0.1](1.986875,0.22640625)
\psdots[dotsize=0.1](2.586875,-0.27359375)
\psdots[dotsize=0.1](2.586875,0.22640625)
\psdots[dotsize=0.1](2.286875,0.7264063)
\psline[linewidth=0.03cm](2.286875,0.7264063)(1.986875,0.22640625)
\psline[linewidth=0.03cm](2.586875,0.22640625)(2.586875,-0.27359375)
\psline[linewidth=0.03cm](1.986875,-0.27359375)(1.986875,0.22640625)
\psline[linewidth=0.03cm](1.986875,-0.27359375)(2.586875,-0.27359375)
\psline[linewidth=0.03cm](2.586875,0.22640625)(2.286875,0.7264063)
\psline[linewidth=0.03cm](1.986875,0.22640625)(2.586875,0.22640625)
\usefont{T1}{ptm}{b}{n}
\rput(0.57984376,-0.66859376){\small $Chair$}
\psdots[dotsize=0.1](3.786875,0.22640625)
\psdots[dotsize=0.1](4.086875,-0.27359375)
\psdots[dotsize=0.1](4.386875,0.22640625)
\psdots[dotsize=0.1](3.786875,0.7264063)
\psdots[dotsize=0.1](4.386875,0.7264063)
\psline[linewidth=0.03cm](3.786875,0.7264063)(3.786875,0.22640625)
\psline[linewidth=0.03cm](3.786875,0.22640625)(4.086875,-0.27359375)
\psline[linewidth=0.03cm](4.086875,-0.27359375)(4.386875,0.22640625)
\psline[linewidth=0.03cm](4.386875,0.22640625)(3.786875,0.22640625)
\psline[linewidth=0.03cm](4.386875,0.22640625)(4.386875,0.7264063)
\psdots[dotsize=0.1](5.886875,0.7264063)
\psdots[dotsize=0.1](5.586875,0.42640626)
\psdots[dotsize=0.1](6.186875,0.42640626)
\psdots[dotsize=0.1](5.886875,0.12640625)
\psdots[dotsize=0.1](5.886875,-0.27359375)
\psline[linewidth=0.03cm](5.886875,0.7264063)(6.186875,0.42640626)
\psline[linewidth=0.03cm](6.186875,0.42640626)(5.886875,0.12640625)
\psline[linewidth=0.03cm](5.886875,0.12640625)(5.886875,0.7264063)
\psline[linewidth=0.03cm](5.886875,0.7264063)(5.586875,0.42640626)
\psline[linewidth=0.03cm](5.586875,0.42640626)(5.886875,0.12640625)
\psline[linewidth=0.03cm](5.886875,0.12640625)(5.886875,-0.27359375)
\psdots[dotsize=0.1](7.586875,0.7264063)
\psdots[dotsize=0.1](7.286875,0.42640626)
\psdots[dotsize=0.1](7.886875,0.42640626)
\psdots[dotsize=0.1](7.586875,0.12640625)
\psdots[dotsize=0.1](7.586875,-0.27359375)
\psline[linewidth=0.03cm](7.586875,0.7264063)(7.886875,0.42640626)
\psline[linewidth=0.03cm](7.886875,0.42640626)(7.586875,0.12640625)
\psline[linewidth=0.03cm](7.586875,0.7264063)(7.286875,0.42640626)
\psline[linewidth=0.03cm](7.286875,0.42640626)(7.586875,0.12640625)
\psline[linewidth=0.03cm](7.586875,0.12640625)(7.586875,-0.27359375)
\psline[linewidth=0.03cm](7.286875,0.42640626)(7.886875,0.42640626)
\usefont{T1}{ptm}{b}{n}
\rput(2.3098438,-0.66859376){\small $House$}
\usefont{T1}{ptm}{b}{n}
\rput(3.9798439,-0.66859376){\small $Bull$}
\usefont{T1}{ptm}{b}{n}
\rput(5.7898436,-0.66859376){\small $Dart$}
\usefont{T1}{ptm}{b}{n}
\rput(7.469844,-0.66859376){\small $Kite$}
\end{pspicture} 
}
\caption{Configurations Chair, House, Bull, Dart,Kite}
\label{fig:ChairHouseBullDartKite}

\end{figure}


